Sparse Probabilistic Circuits via Pruning and Growing

Probabilistic circuits (PCs) are a tractable representation of probability distributions allowing for exact and efficient computation of likelihoods and marginals. There has been significant recent progress on improving the scale and expressiveness of PCs. However, PC training performance plateaus as model size increases. We discover that most capacity in existing large PC structures is wasted: fully-connected parameter layers are only sparsely used. We propose two operations: pruning and growing, that exploit the sparsity of PC structures. Specifically, the pruning operation removes unimportant sub-networks of the PC for model compression and comes with theoretical guarantees. The growing operation increases model capacity by increasing the size of the latent space. By alternatingly applying pruning and growing, we increase the capacity that is meaningfully used, allowing us to significantly scale up PC learning. Empirically, our learner achieves state-of-the-art likelihoods on MNIST-family image datasets and on Penn Tree Bank language data compared to other PC learners and less tractable deep generative models such as flow-based models and variational autoencoders (VAEs).

==> tikzlibrarypc.code.tex <==

\usetikzlibrary{chains}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usepackage{xparse}


\newdimen\mywidth
\newdimen\myheight

\newcommand*{\IfStringInList}[2]{%
  \in@{,#1,}{,#2,}%
  \ifin@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}


\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}


\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodeleft}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodedown}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {#3};
}

\newcommand{\cbernodedown}[4][]{
  \node[circle,fill=white,draw=#4,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw[draw=#4] circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {\textcolor{#4}{#3}};
}

\DeclareDocumentCommand{\contnode}{o m m o}  
{%
  \IfNoValueTF{#4}
  {\contnodebelow[#1]{#2}{#3}}
  {\contnodeleft[#1]{#2}{#3}}
}

\newcommand{\contnodebelow}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture}
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnodeleft}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} 
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


\newcommand{\edge}[3][]{ %
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\cedge}[3][]{ %
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[-,#1] (\x)+(0,-9pt) -- ($(0,9pt)+(\y)$);
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}

\newcommand{\colorweigedge}[7][]{
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;
      \pgfmathparse{width("\noexpand\noexpand\noexpand#4")} ; %
      \pgfmathsetlength{\mywidth}{\pgfmathresult} ; %
      \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %
      \pgfmathsetlength{\myheight}{\pgfmathresult} ; %
      \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#6,text=#7,minimum height=1.8\myheight,minimum width=1.2\mywidth,label={center:\textcolor{#7}{#4}}] at ($(\x)!0.5!(\y)$) {} ;
    } ;
  } ;
}

\newcommand{\ellipsis}[2]{
  \node at ($(#1)!.5!(#2)$) {\ldots} ;
}

\newcommand{\annotatenode}[4]{
  \node[] at ([xshift=#3,yshift=#4]#1) {#2} ;
}

\newcommand{\colorfulannotnode}[6]{
  \pgfmathparse{width("\noexpand\noexpand\noexpand#2")} ; %
  \pgfmathsetlength{\mywidth}{\pgfmathresult} ; %
  \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %
  \pgfmathsetlength{\myheight}{\pgfmathresult} ;
  \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#5,text=#6,minimum height=1.3\myheight,minimum width=1.3\mywidth,label={center:\textcolor{#6}{#2}}] at ([xshift=#3,yshift=#4]#1) {} ;
}

\newcommand{\midlinewidth}{1.0pt}
\newcommand{\incmidlinewidth}{1.7pt}
\newcommand{\largelinewidth}{1.9pt}
\newcommand{\xlargelinewidth}{2.3pt}
\newcommand{\middist}{17pt}
\newcommand{\sqintermiddist}{15.5pt}
\newcommand{\intermiddist}{30pt}
\newcommand{\largedist}{49pt}
\newcommand{\midsmalldist}{10pt}
\newcommand{\smalldist}{6pt}
\newcommand{\tinydist}{4pt}
\newcommand{\centraldist}{30pt}
\newcommand{\midlargedist}{24pt}
\newcommand{\halfdist}{19pt}
\newcommand{\weightsize}{\fontsize{10}{10}\selectfont}
\newcommand{\annotsize}{\fontsize{10}{10}\selectfont}

\definecolor{lacamlilac} {RGB} {107,93,153}
\definecolor{lacamlilac2} {RGB} {93, 109, 152}
\definecolor{lacamlightlilac} {RGB} {174, 166, 201}
\definecolor{lacamdarklilac} {RGB} {51, 10, 102}
\definecolor{lacamdarklilac5} {RGB} {51, 10, 102}
\colorlet{lacamdarklilac4} {lacamdarklilac5!80!}
\colorlet{lacamdarklilac3} {lacamdarklilac5!60!}
\colorlet{lacamdarklilac2} {lacamdarklilac5!40!}
\colorlet{lacamdarklilac1} {lacamdarklilac5!20!}

\definecolor{lacamgold5} {RGB} {255, 87, 0}
\colorlet{lacamgold4} {lacamgold5!80!}
\colorlet{lacamgold3} {lacamgold5!60!}
\colorlet{lacamgold2} {lacamgold5!40!}
\colorlet{lacamgold1} {lacamgold5!20!}
\definecolor{violet} {RGB} {119, 111, 178}
\definecolor{petroil2} {RGB} {36, 165, 175}
\definecolor{petroil4} {RGB} {30, 132, 149}
\definecolor{petroil6} {RGB} {23, 101, 115}
\definecolor{gold2} {RGB} {255, 130, 0}
\definecolor{gold4} {RGB} {250, 100, 0}
\definecolor{gold6} {RGB} {245, 90, 0}

\definecolor{lacamoil5}{rgb}{0.13, 0.67, 0.8}
\colorlet{lacamoil4} {lacamoil5!80!}
\colorlet{lacamoil3} {lacamoil5!60!}
\colorlet{lacamoil2} {lacamoil5!40!}
\colorlet{lacamoil1} {lacamoil5!20!}

\definecolor{lightgray} {RGB} {210, 210, 210}
\definecolor{myblue} {RGB} {80, 145, 207}
\definecolor{mypurple} {RGB} {101, 43, 150}
\definecolor{myred} {RGB} {255, 0, 1}

\definecolor{tomato0} {HTML} {EF9A9A}
\definecolor{tomato1} {HTML} {F44336}
\definecolor{tomato2} {HTML} {E53935}
\definecolor{tomato3} {HTML} {D32F2F}
\definecolor{tomato4} {HTML} {C62828}
\definecolor{tomato5} {HTML} {B71C1C}


\definecolor{peas1} {HTML} {009688}
\definecolor{peas2} {HTML} {00897B}
\definecolor{peas3} {HTML} {00796B}
\definecolor{peas4} {HTML} {00695C}
\definecolor{peas5} {HTML} {004D40}

\definecolor{bgrey0} {HTML} {78909C}
\definecolor{bgrey1} {HTML} {607D8B}
\definecolor{bgrey2} {HTML} {546E7A}
\definecolor{bgrey3} {HTML} {455A64}
\definecolor{bgrey4} {HTML} {37474F}
\definecolor{bgrey5} {HTML} {263238}

\definecolor{olive0} {HTML} {C5E1A5}
\definecolor{olive1} {HTML} {AED581}
\definecolor{olive2} {HTML} {9CCC65}
\definecolor{olive3} {HTML} {8BC34A}
\definecolor{olive4} {HTML} {7CB342}
\definecolor{olive5} {HTML} {689F38}

\definecolor{pink0} {HTML} {FCE4EC}
\definecolor{pink1} {HTML} {F8BBD0}
\definecolor{pink2} {HTML} {F48FB1}
\definecolor{pink3} {HTML} {F06292}
\definecolor{pink4} {HTML} {EC407A}
\definecolor{pink5} {HTML} {FF80AB}

\definecolor{brown0} {HTML} {D7CCC8}
\definecolor{brown1} {HTML} {BCAAA4}
\definecolor{brown2} {HTML} {A1887F}
\definecolor{brown3} {HTML} {8D6E63}
\definecolor{brown4} {HTML} {795548}
\definecolor{brown5} {HTML} {6D4C41}
\definecolor{brown6} {HTML} {5D4037}

\definecolor{yellow0} {HTML} {CDDC39}
\definecolor{yellow1} {HTML} {9E9D24}
\definecolor{yellow3} {HTML} {FFBD2A}
\definecolor{yellow4} {HTML} {FFB000}
\definecolor{yellow5} {HTML} {FFD600}


